Lattice computation of the Kugo-Ojima correlation function

As of today, color confinement in Quantum Chromodynamics remains a mystery from the theoretical point of view. So far, no analytical proof of color confinement has been found and the mechanism that confines colored states from the space of physical states is still unknown. Taichiro Kugo and Izumi Ojima proposed such confinement mechanism, using as basis the BRST-symmetry and derived the requirements for the realization of this mechanism. One such requirement, which happens to be the non-trivial one, is that a special correlation function, the Kugo-Ojima correlation function $u(p^2)$, approaches $-1$ at the origin ($p^2=0)$. This correlation function can be obtained on the lattice within the lattice formulation of gauge theories. The present work consists on lattice results for this correlation function on the Landau gauge. We present results obtained from 4 symmetric large volume lattices $(32^{4}, 48^{4}, 64^{4}, 80^{4})$ with $\beta = 6.0$ on the Landau gauge. A test on the transversality of the Kugo-Ojima correlation function is also performed, along with some statistical considerations of the results. The results present further evidence that the Kugo-Ojima confinement scenario is not realized on the lattice and that the Kugo-Ojima correlation function, in the Landau gauge, is transverse. Our findings align qualitatively with existing literature.

==> list_acronyms.tex <==
\begin{acronym}[PROJECT\_NAME]
    \acro{DEA}{Dissertation's Example Acronym}
    \acro{QCD}{Quantum Chromodynamics}
\end{acronym}

